Classification via Incoherent Subspaces

This article presents a new classification framework that can extract individual features per class. The scheme is based on a model of incoherent subspaces, each one associated to one class, and a model on how the elements in a class are represented in this subspace. After the theoretical analysis an alternate projection algorithm to find such a collection is developed. The classification performance and speed of the proposed method is tested on the AR and YaleB databases and compared to that of Fisher's LDA and a recent approach based on on $\ell_1$ minimisation. Finally connections of the presented scheme to already existing work are discussed and possible ways of extensions are pointed out.

==> jp for arxiv/makros.tex <==
%
% Makros for Classification Paper
%

\newcommand\eps{{\varepsilon}}

\newcommand\sig{{y}}
\newcommand\signew{{\sig_{new}}}
\newcommand\class{{Y}}
\newcommand\X{{\class}}
\newcommand\A{{A}}
\newcommand\Abest{{A^{best}}}
\newcommand\Sens{{S}}
\newcommand\nsens{{s}}
\newcommand\coef{x}

\newcommand\feat{{f}}
\newcommand\featnew{{\feat_{new}}}
\newcommand\F{{F}}
\newcommand\Feat{{F}}
\newcommand\Fn{{F}}
\newcommand\fn{{f}}
\newcommand\rk{{\operatorname{rk}}}
\newcommand\sign{{\operatorname{sign}}}
\newcommand\prox{{\operatorname{prox}}}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\newcommand\ip[2]{\langle #1, #2\rangle}
\newcommand\atom{{\varphi}}

\newcommand\nsig{{N}}
\newcommand\ddim{{d}}
\newcommand\nproj{{p}}
\newcommand\nclass{{c}}
\newcommand\n{{n}}
\newcommand\nf{{s}}

\newcommand\Gram{{G}}
\newcommand\Gbest{G^{best}}

\newcommand{\R}{{\mathbb{R}}}
\newcommand{\Z}{{\mathbb{Z}}}
\newcommand{\C}{{\mathbb{C}}}

\newcommand{\ie}{{i.e. }}

%\theoremstyle{plain}
\newtheorem{Theorem}{Theorem}
\newtheorem{lemma}[Theorem]{Lemma}
\newtheorem{corollary}[Theorem]{Corollary}
\newtheorem{example}[Theorem]{Example}
\newtheorem{proposition}[Theorem]{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{conj}[Theorem]{Conjecture}

%\theoremstyle{remark}
%\newtheorem{remark}{Remark}

\newenvironment{Proof}{\noindent
{\bf{Proof:} }}
{\hspace*{\fill}\qed\vskip1em}

